A path towards constraining the evolution of the interstellar medium and outflows in the Milky Way using APOGEE

In recent years, the study of the Milky Way has significantly advanced due to extensive spectroscopic surveys of its stars, complemented by astroseismic and astrometric data. However, it remains disjoint from recent advancements in understanding the physics of the Galactic interstellar medium (ISM). This paper introduces a new model for the chemical evolution of the Milky Way that can be constrained on stellar data, because it combines a state-of-the-art ISM model with a Milky Way stellar disc model. Utilizing a dataset of red clump stars from APOGEE, known for their precise ages and metallicities, we concentrate on the last 6 billion years -- a period marked by Milky Way's secular evolution. We examine the oxygen abundance in the low-$\alpha$ disc stars relative to their ages and birth radii, validating or constraining critical ISM parameters that remain largely unexplored in extragalactic observations. The models that successfully reproduce the radius -- metallicity distribution and the age -- metallicity distribution of stars without violating existing ISM observations indicate a need for modest differential oxygen enrichment in Galactic outflows, meaning that the oxygen abundance of outflows is higher than the local ISM abundance, irrespective of outflow mass loading. The models also suggest somewhat elevated ISM gas velocity dispersion levels over the past 6 billion years compared to galaxies of similar mass. The extra turbulence necessary could result from energy from gas accretion onto the Galaxy, supernovae clustering in the ISM, or increased star formation efficiency per freefall time. This work provides a novel approach to constraining the Galactic ISM and outflows, leveraging the detailed insights available from contemporary Milky Way surveys.

==> gm2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% The caption of this graphical model
% is at the bottom of the page
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{shapes,arrows,positioning,fit,decorations.pathreplacing,calligraphy}

%\usetikzlibrary{shapes,arrows,positioning,fit}

\begin{figure*}
\centering
%
% Start the graphical model
%
\begin{tikzpicture} %[>=stealth']


% define colors
\definecolor{bblue}{RGB}{34,94,168}
\definecolor{ggreen}{RGB}{35,132,67}
\definecolor{rm}{RGB}{140,45,4}

%---------------------------------------
% Make some commands
%---------------------------------------
\tikzstyle{main}=[circle, minimum size = 12mm, line width=0.4mm, draw =black!80, node distance = 7mm]
\tikzstyle{ellip}=[ellipse, minimum width=10mm, minimum height=5mm), line width=0.4mm, draw =black!80, node distance = 7mm]
\tikzset{err/.style={
    rectangle,
    minimum size=2mm,
    thick,
    draw=black!100,
    node distance=9mm
}}
\tikzstyle{errc}=[circle, minimum size = 2mm, thick, draw =black!100, node distance = 9mm]

\tikzstyle{connect}=[-latex, thick, ->]
\tikzstyle{box}=[rectangle, draw=black!100]
\tikzstyle{line}=[draw]


%-----------------------------------------
% Make Nodes
%-----------------------------------------
   % 0th floor = observables
   \node[ellip, minimum width=7mm, fill = black!15] (xv) [align=center]{$R_{\mathrm{gal},i}$\\ $z_{\mathrm{gal},i}$};
   %\node[ellip, minimum width=9mm, fill=black!15] (v) [left=of xv, align=center]{$v_{Ri}$\\ $v_{\phi i}$};
   \node[ellip, minimum width=25mm,fill = black!15] (feobs) [right=of xv, align=center]{[O/H]$_{\mathrm{obs}\,i}$};
   \node[main, fill = black!15] (tobs) [right=5mm of feobs, label=center:$\tau_{\mathrm{obs}\,i}$] { };
   
   
   % 1st floor: action and metallicity
   %\node[main, fill=white!100](J)[above=of xv, label=center:{$\boldsymbol{J}_i, \boldsymbol{\theta}_i$}] {};
   \node[main, fill=white!100](fe)[above=of feobs, label=center:{[O/H]$_i$}] {};   
   \coordinate (OHnode) at ([xshift=4.5cm]fe.west);

   % 2nd floor: birth conditions: birth angular momentum, age
   \node[main, fill=white!100](Lz0)[above=20mm of xv, label=center:{$R$}] {};
   \node[main, fill=white!100](t)[right=37mm of Lz0, label=center:{$\tau_i$}] {};

   \node[ellip, minimum width=28mm, fill = black!15] (evol) [right=of t][draw, align=center] {Evolutionary  \\stage $i$ };

   % 3rd floor: birth parameters
   \node[errc, fill=black!100](Rd0)[above=10mm of Lz0, label=above:structure]{};
   \node[above=2mm of Rd0, label=above:Formation, align=center] {};
   %{Formation\\ structure, $R_{d0}$};   
 
   \node[errc, fill=black!100](SFH)[right=46.5mm of Rd0, label=above:history]{};
   \node[above=2mm of SFH, label=above:Star formation, align=center] {};

   % Left:  Potential and secular evolution
   \node[errc, fill=black!100](secular)[left=35mm of fe, label={[align=center]left: Secular \\evolution}]{}; 

   \node[errc, fill=black!100](errt)[right=54mm of tobs, label=below:$\sigma_{\tau}$] {};
   
   % selection function
   \node[errc, fill=black!100](selfunc)[left=8mm of xv, label={[align=center]left: APOGEE \\spatial selection}]{};
   \node[errc, fill=black!100](RC)[right=55mm of t, label={[align=center]below: Red Clump\\ selection}]{};

   \node[errc, fill=black!100](errfe)[below=10mm of feobs, label=below:$\sigma_{[\mathrm{O}/\mathrm{H}]}$] {}; 

   % Potential
   \node[errc, fill=black!100](pot)[left=22.75mm of errfe, label=left:Potential] {};

   % Rectangle around single objects to take the product over
   \node[rectangle, fit= (Lz0) (evol) (xv), label={[xshift=46mm]above:{$ i=1,...,N $}}] (rect) {};
   \node[rectangle, fit=(rect), inner sep=4.5mm, draw=black!100] {};



%-----------------------------------------
% Make Nodes
%-----------------------------------------
   % 0th floor = Mg, sigmag
   \node[ellip, fill = white!100, draw=ggreen] (Mg) [below right = 7.7cm and 70mm of secular, align=center, line width=0.8mm] {Mass \\ balance \\ $M_{\rm{g}}$};
   
   % 1st floor: physical processes and PSA
   \node[ellip, fill=white!100] (radialflows) [above left = 10mm and 20mm of Mg, align=center] {Radial \\ gas flows};
   
   \node[ellip, fill=white!100](starformation)[below=9mm of radialflows][align=center]{Star \\ formation};
   \node[ellip, fill=white!100](starformationparams)[left=5mm of starformation][align=center]{$f_{\rm{sf}},\,\epsilon_{\rm{ff}},\,f_{\rm{gQ}}$ \\ $\sigma_{\rm{SF}},\,C_{\rm{SN}},\,t_{\rm{sf,max}}$};

   \node[ellip, fill=white!100] (radialflowsparams) [above=10mm of starformationparams][align=center] {$\phi_{\rm{nt}},\,F\,(\sigma_{\rm{g}})$};

   \node[ellip, fill=white!100](winds)[below=6mm of starformation][align=center]{Galactic \\ winds};
   \node[ellip, fill=white!100](windsparams)[below=7mm of starformationparams][align=center]{$\phi_{\rm{y}},\,\eta_{\rm{w}},\,\mathcal{Z}_{\rm{w}}$};
   
  
   \node[ellip, fill=white!100](accretion)[below=3mm of winds][align=center]{Gas \\ accretion};
   \node[ellip, fill=white!100](accretionparams)[below=19mm of starformationparams][align=center]{$\dot M_{\rm{g,acc}},\,\epsilon_{\rm{in}},\,c$ \\ $\sigma_{\rm{acc}},\,\xi_{\rm{a}}$};
   
   \node[ellip, fill=white!100](diffusion)[above right=0.mm and 5mm of Mg][align=center]{Metal \\ Diffusion};
   \node[main, fill=white!100] (P) [right=6mm of diffusion][draw, align=center] {$\mathcal{P}$};
   \node[main, fill=white!100] (A) [right=55mm of accretion][draw, align=center] {$\mathcal{A}$ };
   \node[main, fill=white!100] (S) [right=55mm of winds][draw, align=center] {$\mathcal{S}$ };
   

    % Left: toomre Q and hydrostatic eqbm
   \node[errc, fill=black!100](tQ)[above left=2mm and 14 mm of radialflows, label=left:Toomre $Q$]{};
   \node[ellip, fill=white!100](toomreQparams)[below=2mm of radialflowsparams, align=center] {$\phi_{\rm{Q}}$};

   \node[ellip, fill=white!100, line width=0.8mm, draw=ggreen](hydrostat)[above = 20 mm of diffusion, align=center]{Hydrostatic \\ equilibrium};
   \node[ellip, fill=white!100](hydrostatparams)[left = 55 mm of hydrostat, align=center]{$\eta,\,f_{\rm{gP}},\,\phi_{\rm{mp}}$};
   %\node[left=7mm of hydrostat, label=above:Hydrostatic, align=center] {};

   
   \node[errc, fill=black!100](y)[right=21mm of S, label=below:Yield]{};
   \node[below=8mm of y, label=above:$y$, align=center] {};


   \node[ellip, fill=white!100, line width=0.8mm, draw=ggreen](energybalance)[above=6mm of Mg][draw, align=center]{Energy \\ balance \\ $\sigma_{\rm{g}}$};
   \coordinate (energynode) at ([xshift=6.5cm]energybalance.west);

  
\draw[thick] (OHnode) -- (fe);
\draw[-,thick] (energynode) -- (OHnode);

%\draw[thick] (Jnode) -- (xv);

%\draw[decorate,decoration={calligraphic brace,amplitude=10mm,mirror, segment length=0pt}]([xshift=-9mm, yshift=1mm]hydrostatparams.north west) -- node[midway, left=10mm] {ISM} ([xshift=-7mm, yshift=-1mm]accretionparams.south west);
\draw[decorate,decoration={calligraphic brace,amplitude=10mm,mirror, segment length=0pt}] ([xshift=-9mm, yshift=1mm] hydrostatparams.north west) -- node[midway, left=10mm, font=\large] {ISM} ([xshift=-7mm, yshift=-1mm] accretionparams.south west);


\draw[decorate,decoration={calligraphic brace,amplitude=10mm, segment length=0pt}]([xshift=5mm, yshift=12mm]RC.north east) -- node[midwayy, right=10mm, font=\large] {Stars} ([xshift=5mm, yshift=-12mm]errt.south east);


%\draw [decorate,decoration={brace,amplitude=16mm,mirror}] (hydrostatparams.north west) -- (accretionparams.south west) node [black,midway,xshift=-1.5cm] {};

        
%\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=2mm},yshift=0pt] (hydrostatparams.east) -- (accretionparams.west) node[midway, below=7mm, align=center] {Range of\\parameters};


%\node [callout,brace=(hydrostatparams) to (accretionparams),callout pointer arc=30pt,yshift=-5mm] {Range of parameters};


%------------------------------------------------
% Draw the connections
%------------------------------------------------

  \path     (Rd0) edge [connect] (Lz0)
		(Lz0) edge [connect, bend left=20] (t)
		(SFH) edge [connect] (t)
		%(pot) edge [connect] (v)
            %(Lz0) edge [connect] (v)
            %(secular) edge [connect] (v)
            (pot) edge [connect] (xv)
		(Lz0) edge [connect] (xv)
		(Lz0) edge [connect] (fe)
		(t) edge [connect, bend right=35] (xv)
		(t) edge [connect] (fe)
		(t) edge [connect] (evol)
		(t) edge [connect] (tobs)
            (secular) edge [connect] (xv)
		%(J) edge [connect] (xv)
		%(J) edge [connect] (v)
		(fe) edge [connect] (feobs)
		%(errdyn) edge [connect] (v)
		(errfe) edge [connect] (feobs)
		(errt) edge [connect] (tobs)
		(selfunc) edge [connect] (xv)
		(RC) edge [connect] (evol)
            %ism:
            (y) edge [connect] (S)
            (P) edge [-, thick, bend right=45] (energynode)
            (S) edge [-, thick, bend right=45] (energynode)
            (A) edge [-, thick, bend right=45] (energynode)
		(Mg) edge [connect] (accretion)
		(Mg) edge [connect] (starformation)
		(Mg) edge [connect] (winds)
		(Mg) edge [connect] (radialflows)
		(accretion) edge [connect] (Mg)
		(radialflows) edge [connect] (Mg)
		(starformation) edge [connect] (Mg)
		(winds) edge [connect] (Mg)
		(energybalance) edge [connect] (starformation)
		(energybalance) edge [connect] (diffusion)
		(energybalance) edge [connect] (radialflows)
		%(R0) edge [connect] (chemical)
		%(ZR0) edge [connect] (chemical)
		%(S) edge [connect] (ZR0)
		%(A) edge [connect] (ZR0)
		(diffusion) edge [connect] (P)
		(diffusion) edge [connect] (S)
		(diffusion) edge [connect, bend right =20] (A)
		(radialflows) edge [connect, bend left=50] (P)
		(accretion) edge [connect] (A)
		(starformation) edge [connect, bend right=40] (S)
		(winds) edge [connect] (S)
		(tQ) edge [connect] (starformation)
		(tQ) edge [connect] (radialflows)
		(hydrostat) edge [connect] (diffusion)
		(hydrostat) edge [connect] (radialflows)
		%(hydrostat) edge [connect] (starformation)
		(starformation) edge [connect] (winds)
		%(accretion) edge [connect, bend right=50] (starformation)
		%(accretion) edge [connect, bend right=60] (radialflows);
		(accretionparams) edge [connect] (accretion)
		(starformationparams) edge [connect] (starformation)
		(radialflowsparams) edge [connect] (radialflows)
		(windsparams) edge [connect] (winds)
		(toomreQparams) edge [connect] (radialflows)
		(toomreQparams) edge [connect] (starformation)
		(hydrostatparams) edge [connect] (hydrostat)
            (Mg) edge [connect] (energybalance);
           

% Shift "Mg" node down by 5mm
		
\end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CAPTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Graphical model that shows the different components of the chemical evolution model, with curly braces marking the corresponding stellar and ISM parts. Filled gray circles denote APOGEE observables, solid dots denote parameters that we keep fixed in this work, and colorless ellipses/circles denote parameters we vary. The green ellipses denote the equilibria we consider in the ISM. All the relevant ISM physics (specified by various symbols in bottom left) gets condensed into three key dimensionless ratios -- $\mathcal{P},\,\mathcal{S}$, and $\mathcal{A}$. We use the model to produce synthetic distributions of stars with a given metallicity, current day galactocentric radius, and age that we then compare against APOGEE data. Definitions of all the parameters are listed in \autoref{tab:taball}.}
\label{fig:graphical_model} 
\end{figure*}
